Ponderomotive effects in multiphoton pair production

The Dirac-Heisenberg-Wigner formalism is employed to investigate electron-positron pair production in cylindrically symmetric but otherwise spatially inhomogeneous, oscillating electric fields. The oscillation frequencies are hereby tuned to obtain multiphoton pair production in the nonperturbative threshold regime. An effective mass as well as a trajectory-based semi-classical analysis are introduced in order to interpret the numerical results for the distribution functions as well as for the particle yields and spectra. The results, including the asymptotic particle spectra, display clear signatures of ponderomotive forces.

==> author_list.tex <==

\affiliation{Institut f\"ur Physik, Karl-Franzens-Universit\"at, A-8010 Graz, Austria}
\affiliation{Theoretisch-Physikalisches Institut, Abbe Center of Photonics, Friedrich-Schiller-Universit\"at Jena, D-07743 Jena, Germany}

%
\author{Christian Kohlf\"urst} 
\email{C.Kohlfuerst@gsi.de}
\affiliation{Theoretisch-Physikalisches Institut, Abbe Center of Photonics,
Friedrich-Schiller-Universit\"at Jena, Max-Wien-Platz 1, D-07743 Jena, Germany \\ 
Helmholtz-Institut Jena, Fr\"obelstieg 3, D-07743 Jena, Germany}
\author{Reinhard Alkofer} 
\email{reinhard.alkofer@uni-graz.at}
\affiliation{Institut f\"ur Physik, Karl-Franzens-Universit\"at, A-8010 Graz, Austria}

%\noaffiliation
%
\vskip 0.25cm

